Regret in Online Recommendation Systems

This paper proposes a theoretical analysis of recommendation systems in an online setting, where items are sequentially recommended to users over time. In each round, a user, randomly picked from a population of $m$ users, requests a recommendation. The decision-maker observes the user and selects an item from a catalogue of $n$ items. Importantly, an item cannot be recommended twice to the same user. The probabilities that a user likes each item are unknown. The performance of the recommendation algorithm is captured through its regret, considering as a reference an Oracle algorithm aware of these probabilities. We investigate various structural assumptions on these probabilities: we derive for each structure regret lower bounds, and devise algorithms achieving these limits. Interestingly, our analysis reveals the relative weights of the different components of regret: the component due to the constraint of not presenting the same item twice to the same user, that due to learning the chances users like items, and finally that arising when learning the underlying structure.

==> lower.tex <==
\section{Regret Lower Bounds}\label{sec:lower}


In this section, we derive regret lower bounds for the different structured problems introduced in the previous section. Interestingly, we are able to quantify the minimal regret induced by the specific and individual features of the problem: (i) the no-repetition constraint, (ii) the unknown success probabilities, (iii) the unknown item clusters, (iv) the unknown user clusters. 

\subsection{Clustered items and statistically identical users}

Recall that the success rates $p$ of the different clusters are such that $p_1>p_2\ge p_3\ge \ldots \ge p_K$. We denote by $\Delta_k=p_1-p_k$ the gap between items from the best cluster and items from cluster ${\cal I}_k$. We also introduce the function:
$$
\phi(k,m,p) = {1\over 8} e^{-\gamma(p_1,p_{k})}\times {1- e^{-m \gamma(p_1,p_{k})}\over 1- e^{-\gamma(p_1,p_{k})}},
$$
where $\gamma(p,q)=\kl(p,q)+\kl(q,p)$. Using the fact that $\kl(p,q)\le {(p-q)^2/ q(1-q)}$, we can easily show that as $m$ grows large, $\phi(k,m,p)$ scales as $\eta/(16\Delta_k^2)$ when $\Delta_k$ is small, where $\eta:=\min_kp_k(1-p_k)$. 

We aim at deriving problem-specific rather than minimax regret lower bounds, and as in the classical stochastic bandit literature, we hence need to introduce the notion of {\it uniformly} good algorithm. $\pi$ is uniformly good if its expected regret $R^\pi(T)$ is $O(\max\{ \sqrt{T}, {\log(m)\over \log({m\log(m)\over T}+e)}$ for all possible system parameters $(p,\alpha)$ when $T,m,n$ grows large with $T=o(nm)$ and $m\ge n$. In the next section, we establish that our proposed algorithms are uniformly good. 

\begin{theorem}\label{th:lowA}
Let $\pi\in \Pi$ be an arbitrary algorithm. Then its regret satisfies: for all $T\ge 1$ such that $m\ge c/\Delta_2^2$ (for some constant $c$ large enough)
$$
R^\pi(T) \ge \max\{ R_{\mathrm{nr}}(T), R_{\mathrm{ic}}(T) \},
$$
where $R_{\mathrm{nr}}(T)$ and $R_{\mathrm{ic}}(T)$ are the regrets due to the no-repetition constraint and to the unknown item clusters, respectively, defined by:
$$
\left\{
\arraycolsep=1.2pt\def\arraystretch{1.9}
\begin{array}{l}
R_{\mathrm{nr}}(T) = \mathbb{E}[\max_uN_u]  \sum_{k\neq 1}\alpha_k\Delta_k,\\
R_{\mathrm{ic}}(T) = T \times {\sum_{k\neq 1}\alpha_k \phi(k,m,p)\Delta_k \over \sum_{k\neq 1}\alpha_k \phi(k,m,p) + m\alpha_1}.
\end{array}
\right.
$$

Assume that $\pi$ is uniformly good, then we have\footnote{We write $a\gtrsim b$ if $\lim\inf_{T\to\infty}a/b\ge 1$.}:
$$
R^\pi(T)\gtrsim  R_{\mathrm{sp}}(T):=\log(T) \sum_{k\neq 1} {\Delta_k\over \kl (p_k,p_1)},
$$
where $R_{\mathrm{sp}}(T)$ refers to the regret due to the unknown success probabilities.
\end{theorem}

Before proving the theorem, we check how the regret lower bounds scale in small, medium and large time horizons.

({\it Small horizon}) For $T=o(m\log(m))$, we get $R_{\mathrm{nr}}(T)=\Omega({\log(m)\over \log({m\log(m)\over T})})=\omega({T\over m})=\omega(R_{\mathrm{ic}}(T))$, and $R_{\mathrm{sp}}(T)=\Omega(\log(T))$. The regret arises mainly due to either the no-repetition constraint or the need to learn the success probabilities, depending on the relative values of ${\log(m)\over \log({m\log(m)\over T})}$ and $\log(T)$. For example, when $T=m$, the regret scales at least as $\log(T)$, but in general at least as  $\max\{ {\log(m)\over \log({m\log(m)\over T})}, \log(T)\}$. 

({\it Medium horizon}) For $T=c m\log(m)$, we get $R_{\mathrm{nr}}(T)=\Omega(\log(T))$, $R_{\mathrm{ic}}(T)=\Omega(\log(m))$, $R_{\mathrm{sp}}(T)=\Omega(\log(T))$. The three components of the regret lower bound scales in the same way, and the regret scales at least as $\log(T)$. 
 
({\it Large horizon}) For $T=\omega(m\log(m))$, we get $R_{\mathrm{nr}}(T)=\Omega({T\over m})$, $R_{\mathrm{ic}}(T)=\Omega({T\over m})$, $R_{\mathrm{sp}}(T)=\Omega(\log(T))$. One can easily check that ${T\over m}=\omega(\log(T))$, and hence learning the success probabilities induces a regret negligible compared to that due to the need to learn the item clusters or to deal with the no-repetition constraint. The regret then scales at least as ${T\over m}$.   

{\bf Proof.} Let $\pi\in \Pi$. We first establish that for any $T\ge 1$, $R^\pi(T) \ge R_{\mathrm{nr}}(T)$. Observe that under the no-repetition constraint, the number of items that $\pi$ will select is greater than $\max_uN_u(T)$. Now when an item is selected for the first time, by assumption, it belongs to the sub-optimal cluster ${\cal I}_k$ with probability $\alpha_k$, in which case this initial selection induces an expected regret $\Delta_k=p_1-p_k$. Hence indeed, $R^\pi(T) \ge \mathbb{E}[\max_uN_u]  \sum_{k\neq 1}\alpha_k\Delta_k$.

Next, we prove that $R^\pi(T) \gtrsim R_{\mathrm{sp}}(T)$. This part of the regret arises due to the lack of knowledge of the $p_k$'s. Assume that item clusters are known to the algorithm. The item selection problem reduces to a classical stochastic bandit problem. Using the techniques developed in  \cite{lai1985asymptotically} and recently extended in \cite{garivier2018explore}, we can prove that $R^\pi(T) \gtrsim \log(T) \sum_{k\neq 1} {\Delta_k\over \kl (p_k,p_1)}$. Note that here, we scale the time horizon and the number items (arms) simultaneously, which requires finite-time arguments as those developed in \cite{garivier2018explore}. Refer to the appendix for a complete proof.

Finally, the most involved part of the proof is to lower bound the regret due to the lack of knowledge of the item clusters, i.e., to prove that for $T\ge 1$, $R^\pi(T)\ge R_{\mathrm{ic}}(T)$. To this aim, assume that the success probabilities $p_k$'s are known. Further simplify the problem by relaxing the no-repetition constraint: instead, we just impose that any item cannot be selected more than $m$ times. With these assumptions, an optimal algorithm can be described through a simple stopping rule $\tau$. When a new item is selected, $\tau$ decides whether to select this item further depending on its previously observed rewards. when $\tau$ decides to stop exploring the item, a new item is selected. Let $\mathbb{E}^\tau[N_k]$ denote the expected number of times an item of cluster ${\cal I}_k$ is selected under $\tau$ (of course, $N_k\le m$). The next lemma is the main ingredient of the proof.

\begin{lemma}\label{lem:2arms} We have for any $m\ge c/\Delta_2^2$ and for any $k\neq 1$:      
$$
{\mathbb{E}^\tau[N_k]\over \mathbb{E}^\tau[N_{1}]} \ge  {\phi(k,m,p)\over m}.
$$
\end{lemma}

The constant $c$ in the above lemma is the same as in Theorem \ref{th:lowA}, and is chosen such that when $m\ge c/\Delta_2^2$, then for any $k$, $\phi(k,m,p)\le m$. This choice ensures that the inequality stated in the above lemma makes sense (we know that $\mathbb{E}^\tau[N_k]\le m$).

{\it Proof of Lemma \ref{lem:2arms}.} This results is proved considering a 2-arm bandit problem. The arms have Bernoulli rewards with respective means $p_1$ and $p_k$. The means are known but the arm with the highest mean is unknown. For this bandit problem, we can build an algorithm based on our stopping rule $\tau$ in the following way: we initially pick an arm and play it using the stopping rule $\tau$; we then switch arm and repeat (when we switch to an arm already played in the past, the previous rewards are discarded). We stop the algorithm when we have switched an odd number of times and the number of rounds is larger than $m$. Let $\kappa$ denote the number of stopping rules applied to the two arms. $\kappa$ is a random variable, and Wald's first lemma implies that the regret accumulated before we stop playing is:
$
R^\tau = \Delta_k \mathbb{E}[\kappa]\mathbb{E}^\tau[N_k].
$
Since $\max\{\mathbb{E}^\tau[N_1],\mathbb{E}^\tau[N_k]\}\le m$, $\mathbb{E}[\kappa]\mathbb{E}^\tau[N_{1}]\le 2m$. Hence:
\begin{equation}\label{eq:reg1}
R^\tau = \Delta_k \mathbb{E}[\kappa]\mathbb{E}^\tau[N_k]\le 2m \Delta_k {\mathbb{E}^\tau[N_k]\over \mathbb{E}^\tau[N_{1}]}.
\end{equation}
Observe that by construction, $R^\tau$ corresponds to the regret of our algorithm for a number of rounds larger than $m$ in the 2-arm bandit problem with known average rewards. Regret lower bounds for such bandit problems have been derived in \cite{Bubeck13}. We can actually show that (refer to the appendix for a proof):

\begin{lemma}\label{lem:reg-2arm} We have: $R^\tau \ge {\Delta_k}\phi(k,m,p)$.
\end{lemma}

Combining this lemma to (\ref{eq:reg1}) yields Lemma \ref{lem:2arms}. \ep

We complete the proof of $R^\pi(T)\ge R_{\mathrm{ic}}(T)$ using Lemma \ref{lem:2arms}. We use our optimal stopping rule $\tau$ for the simplified problem where the $p_k$'s are known, and where the no-repetition constraint is simplified. Each time a new item is selected, it belongs to ${\cal I}_k$ w.p. $\alpha_k$ and it is played $\mathbb{E}^\tau[N_k]$ in expectation. thus, the expected regret per round of our optimal algorithm is: ${\sum_{k\neq 1} \alpha_k \mathbb{E}^\tau[N_k]\Delta_k\over \sum_{k} \alpha_k \mathbb{E}^\tau[N_1]}$. We conclude that:
\begin{align*}
R^\pi(T) & \ge T {\sum_{k\neq 1} \alpha_k \mathbb{E}^\tau[N_k]\Delta_k\over \sum_{k} \alpha_k \mathbb{E}^\tau[N_k]}\\
&  \stackrel{(a)}{\ge} T \Delta_2 {\sum_{k\neq 1} \alpha_k \mathbb{E}^\tau[N_k]\over \sum_{k} \alpha_k \mathbb{E}^\tau[N_k]}\\
& \stackrel{(b)}{\ge} T {\sum_{k\neq 1}\alpha_k \phi(k,m,p)\Delta_k \over \sum_{k\neq 1}\alpha_k \phi(k,m,p) + m\alpha_1},
\end {align*}
where the inequality (a) stems from the fact that for any $k\ge 2$, $\Delta_2\le \Delta_k$. (b) is obtained by applying Lemma \ref{lem:2arms} and observing that the function $x\mapsto x/(x+a)$ is increasing for all $a>0$. \ep 


  


==> lower2.tex <==
\section{Regret Lower Bounds}\label{sec:lower}


In this section, we derive regret lower bounds for the different structured problems introduced in the previous section. Interestingly, we are able to quantify the minimal regret induced by the specific and individual features of the problem: (i) the no-repetition constraint, (ii) the unknown success probabilities, (iii) the unknown item clusters, (iv) the unknown user clusters. 

\subsection{Clustered items and statistically identical users}

Recall that the success rates $p$ of the different clusters are such that $p_1>p_2\ge p_3\ge \ldots \ge p_K$. We denote by $\Delta_k=p_1-p_k$ the gap between items from the best cluster and items from cluster ${\cal I}_k$. We also introduce the function:
$$
\phi(k,m,p) = {1\over 8} e^{-\gamma(p_1,p_{k})}\times {1- e^{-m \gamma(p_1,p_{k})}\over 1- e^{-\gamma(p_1,p_{k})}},
$$
where $\gamma(p,q)=\kl(p,q)+\kl(q,p)$. Using the fact that $\kl(p,q)\le {(p-q)^2/ q(1-q)}$, we can easily show that as $m$ grows large, $\phi(k,m,p)$ scales as $\eta/(16\Delta_k^2)$ when $\Delta_k$ is small, where $\eta:=\min_kp_k(1-p_k)$. 

We aim at deriving problem-specific rather than minimax regret lower bounds, and as in the classical stochastic bandit literature, we hence need to introduce the notion of {\it uniformly} good algorithm. $\pi$ is uniformly good if its expected regret $R^\pi(T)$ is $O(\max\{ \sqrt{T}, {\log(m)\over \log({m\log(m)\over T}+e)})$ for all possible system parameters $(p,\alpha)$ when $T,m,n$ grows large with $T=o(nm)$ and $m\ge n$. In the next section, we establish that our proposed algorithms are uniformly good. 

\begin{theorem}\label{th:lowA}
Let $\pi\in \Pi$ be an arbitrary algorithm. Then its regret satisfies: for all $T\ge 1$ such that $m\ge c/\Delta_2^2$ (for some constant $c$ large enough),
$$
R^\pi(T) \ge \max\{ R_{\mathrm{nr}}(T), R_{\mathrm{ic}}(T) \},
$$
where $R_{\mathrm{nr}}(T)$ and $R_{\mathrm{ic}}(T)$ are the regrets due to the no-repetition constraint and to the unknown item clusters, respectively, defined by:
$$
\left\{
\arraycolsep=1.2pt\def\arraystretch{1.9}
\begin{array}{l}
R_{\mathrm{nr}}(T) = \mathbb{E}[\max_uN_u(T)]  \sum_{k\neq 1}\alpha_k\Delta_k,\\
R_{\mathrm{ic}}(T) = {T\over m} \sum_{k\neq 1}\alpha_k \phi(k,m,p)\Delta_k.
\end{array}
\right.
$$

Assume that $\pi$ is uniformly good, then we have\footnote{We write $a\gtrsim b$ if $\lim\inf_{T\to\infty}a/b\ge 1$.}:
$$
R^\pi(T)\gtrsim  R_{\mathrm{sp}}(T):=\log(T) \sum_{k\neq 1} {\Delta_k\over \kl (p_k,p_1)},
$$
where $R_{\mathrm{sp}}(T)$ refers to the regret due to the unknown success probabilities.
\end{theorem}

Before proving the theorem, let us see how the regret lower bounds scale for small, medium and large time horizons.

({\it Small horizon}) For $T=o(m\log(m))$, we get $R_{\mathrm{nr}}(T)=\Omega({\log(m)\over \log({m\log(m)\over T})})=\omega({T\over m})=\omega(R_{\mathrm{ic}}(T))$, and $R_{\mathrm{sp}}(T)=\Omega(\log(T))$. The regret arises mainly due to either the no-repetition constraint or the need to learn the success probabilities, depending on the relative values of ${\log(m)\over \log({m\log(m)\over T})}$ and $\log(T)$. For example, when $T=m$, the regret scales at least as $\log(T)$, but in general at least as  $\max\{ {\log(m)\over \log({m\log(m)\over T})}, \log(T)\}$. 

({\it Medium horizon}) For $T=c m\log(m)$, we get $R_{\mathrm{nr}}(T)=\Omega(\log(T))$, $R_{\mathrm{ic}}(T)=\Omega(\log(m))$, $R_{\mathrm{sp}}(T)=\Omega(\log(T))$. The three components of the regret lower bound scales in the same way, and the regret scales at least as $\log(T)$. 
 
({\it Large horizon}) For $T=\omega(m\log(m))$, we get $R_{\mathrm{nr}}(T)=\Omega({T\over m})$, $R_{\mathrm{ic}}(T)=\Omega({T\over m})$, $R_{\mathrm{sp}}(T)=\Omega(\log(T))$. One can easily check that ${T\over m}=\omega(\log(T))$, and hence learning the success probabilities induces a regret negligible compared to that due to the need to learn the item clusters or to deal with the no-repetition constraint. The regret then scales at least as ${T\over m}$.   

{\bf Proof.} Let $\pi\in \Pi$. We first establish that for any $T\ge 1$, $R^\pi(T) \ge R_{\mathrm{nr}}(T)$. Observe that under the no-repetition constraint, the number of items that $\pi$ will select is greater than $\max_uN_u(T)$. Now when an item is selected for the first time, by assumption, it belongs to the sub-optimal cluster ${\cal I}_k$ with probability $\alpha_k$, in which case this initial selection induces an expected regret $\Delta_k=p_1-p_k$. Hence indeed, $R^\pi(T) \ge \mathbb{E}[\max_uN_u]  \sum_{k\neq 1}\alpha_k\Delta_k$.

Next, we prove that $R^\pi(T) \gtrsim R_{\mathrm{sp}}(T)$. This part of the regret arises due to the lack of knowledge of the $p_k$'s. Assume that item clusters are known to the algorithm. The item selection problem reduces to a classical stochastic bandit problem. Using the techniques developed in  \cite{lai1985asymptotically} and recently extended in \cite{garivier2018explore}, we can prove that $R^\pi(T) \gtrsim \log(T) \sum_{k\neq 1} {\Delta_k\over \kl (p_k,p_1)}$. Note that here, we scale the time horizon and the number items (arms) simultaneously, which requires finite-time arguments as those developed in \cite{garivier2018explore}. Refer to the appendix for a complete proof.

Finally, the most involved part of the proof is to lower bound the regret due to the lack of knowledge of the item clusters, i.e., to prove that for $T\ge 1$, $R^\pi(T)\ge R_{\mathrm{ic}}(T)$. To this aim, assume that the success probabilities $p_k$'s are known. Further simplify the problem by relaxing the no-repetition constraint: instead, we just impose that any item cannot be selected more than $m$ times. With these assumptions, an optimal algorithm can be described through a simple stopping rule $\tau$. When a new item is selected, $\tau$ decides whether to select this item further depending on its previously observed rewards. when $\tau$ decides to stop exploring the item, a new item is selected. Let $\mathbb{E}^\tau[N_k]$ denote the expected number of times an item of cluster ${\cal I}_k$ is selected under $\tau$ (of course, $N_k\le m$). The next lemma is the main ingredient of the proof.

\begin{lemma}\label{lem:2arms} We have for any $m\ge c/\Delta_2^2$ and for any $k\neq 1$:      
$$
{\phi(k,m,p)\over m}\le {\mathbb{E}^\tau[N_k]\over \mathbb{E}^\tau[N_{1}]} \le 1.
$$
\end{lemma}

The constant $c$ in the above lemma is the same as in Theorem \ref{th:lowA}, and is chosen such that when $m\ge c/\Delta_2^2$, then for any $k$, $\phi(k,m,p)\le m$. This choice ensures that the inequality stated in the above lemma makes sense (we know that $\mathbb{E}^\tau[N_k]\le m$).

{\it Proof of Lemma \ref{lem:2arms}.} This results is proved considering a 2-arm bandit problem. The arms have Bernoulli rewards with respective means $p_1$ and $p_k$. The means are known but the arm with the highest mean is unknown. For this bandit problem, we can build an algorithm based on our stopping rule $\tau$ in the following way: we initially pick an arm and play it using the stopping rule $\tau$; we then switch arm and repeat (when we switch to an arm already played in the past, the previous rewards are discarded). We stop the algorithm when we have switched an odd number of times and the number of rounds is larger than $m$. Let $\kappa$ denote the number of stopping rules applied to the two arms. $\kappa$ is a random variable, and Wald's first lemma implies that the regret accumulated before we stop playing is:
$
R^\tau = \Delta_k \mathbb{E}[\kappa]\mathbb{E}^\tau[N_k].
$
Since $\max\{\mathbb{E}^\tau[N_1],\mathbb{E}^\tau[N_k]\}\le m$, $\mathbb{E}[\kappa]\mathbb{E}^\tau[N_{1}]\le 2m$. Hence:
\begin{equation}\label{eq:reg1}
R^\tau = \Delta_k \mathbb{E}[\kappa]\mathbb{E}^\tau[N_k]\le 2m \Delta_k {\mathbb{E}^\tau[N_k]\over \mathbb{E}^\tau[N_{1}]}.
\end{equation}
Observe that by construction, $R^\tau$ corresponds to the regret of our algorithm for a number of rounds larger than $m$ in the 2-arm bandit problem with known average rewards. Regret lower bounds for such bandit problems have been derived in \cite{Bubeck13}. We can actually show that (refer to the appendix for a proof):

\begin{lemma}\label{lem:reg-2arm} We have: $R^\tau \ge {\Delta_k}\phi(k,m,p)$.
\end{lemma}

Combining this lemma to (\ref{eq:reg1}) yields Lemma \ref{lem:2arms}. \ep

We complete the proof of $R^\pi(T)\ge R_{\mathrm{ic}}(T)$ using Lemma \ref{lem:2arms}. We use our optimal stopping rule $\tau$ for the simplified problem where the $p_k$'s are known, and where the no-repetition constraint is simplified. Each time a new item is selected, it belongs to ${\cal I}_k$ w.p. $\alpha_k$ and it is played $\mathbb{E}^\tau[N_k]$ in expectation. Thus, the expected regret per round of our optimal algorithm is: ${\sum_{k\neq 1} \alpha_k \mathbb{E}^\tau[N_k]\Delta_k\over \sum_{k} \alpha_k \mathbb{E}^\tau[N_1]}$. We conclude that:
\begin{align*}
R^\pi(T) & \ge T {\sum_{k\neq 1} \alpha_k \mathbb{E}^\tau[N_k]\Delta_k\over \sum_{k} \alpha_k \mathbb{E}^\tau[N_k]}\\
&  \stackrel{(a)}{\ge} {T\over m} {\sum_{k\neq 1} \alpha_k \mathbb{E}^\tau[N_1]\phi(k,m,p)\Delta_k \over \sum_{k} \alpha_k \mathbb{E}^\tau[N_1]}\\
& = {T\over m} \sum_{k\neq 1}\alpha_k \phi(k,m,p)\Delta_k,
\end {align*}
where the inequality (a) stems from applying Lemma \ref{lem:2arms} (in the numerator, we use $\mathbb{E}^\tau[N_k]\ge \mathbb{E}^\tau[N_1]{\phi(k,m,p)\over m}$, and in the denominator $\mathbb{E}^\tau[N_k]\le \mathbb{E}^\tau[N_1]$). \ep 

\subsection{Unclustered items and statistically identical users}

To state regret lower bounds, we introduce the function $\psi$ (which is the analogous of function $\phi$ used in the case of clustered items): for any $\mu_1, \mu_2\in [0,1]$,
$$
\psi(\mu_1,\mu_2) = {1\over 8} e^{-\gamma(\mu_1,\mu_{2})}\times {1- e^{-m \gamma(\mu_1,\mu_{2})}\over 1- e^{-\gamma(\mu_1,mu_{k2})}}.
$$ 
We have:

\begin{theorem}\label{th:lowB}
Let $\pi\in \Pi$ be an arbitrary algorithm. Then its regret satisfies: for all $T\ge 1$ such that $m\ge c/\varepsilon^2$ (for some constant $c$ large enough),
$$
R^\pi(T) \ge \max\{ R_{\mathrm{nr}}(T), R_{\mathrm{ic}}(T) \},
$$
where $R_{\mathrm{nr}}(T)$ and $R_{\mathrm{ic}}(T)$ are defined by:
$$
\left\{
\arraycolsep=1.2pt\def\arraystretch{1.9}
\begin{array}{l}
R_{\mathrm{nr}}(T) = \mathbb{E}[\max_uN_u(T)]  \int_0^{\mu_{1-\varepsilon}} (\mu_{1-\varepsilon}-\mu)\zeta(d\mu),\\
R_{\mathrm{ic}}(T) = {T\over m} \int_0^{\mu_{1-\varepsilon}} (\mu_{1-\varepsilon}-\mu)\psi(\mu_{1-{3\over 4}\varepsilon},\mu)\zeta(d\mu).
\end{array}
\right.
$$
\end{theorem}

{\bf Proof.} We apply the same strategy to derive regret lower bound in the case of clustered items. Regarding the regret induced by the no-repetition constraint, we simply get:
$$
R_{\mathrm{nr}}(T) = \mathbb{E}[\max_uN_u(T)]  \int_0^{\mu_{1-\varepsilon}} (\mu_{1-\varepsilon}-\mu)\zeta(d\mu).
$$
Now in absence of clusters, another component of the regret, still denoted by $R_{\mathrm{ic}}(T)$ is due to the lack of knowledge of the success rates of an item when it is first selected, even if the a-priori distribution $\zeta$ is known. Again when $\zeta$ is known, the optimal algorithm boils down to a stopping rule $\tau$ that aims at deciding whether the current item has a success rate greater than $\mu_{1-\varepsilon}$. We denote by $\mathbb{E}^\tau[N_\mu]$ the expected number of rounds an item with success rate $\mu$ is selected under $\tau$. Lemma \ref{lem:2arms} still holds. For two items of respective success rates $\mu_1$ and $\mu_2$ such that $\mu_1-\mu_2\ge \varepsilon/4$, and for $m\ge c/\varepsilon^2$ (with $c$ large enough):
\begin{equation}\label{eq:low2}
{\psi(\mu_1,\mu_2)\over m}\le {\mathbb{E}^\tau[N_{\mu_2}]\over \mathbb{E}^\tau[N_{\mu_1}]} \le 1,
\end{equation} 
Now the regret of an algorithm $\pi$ satisfies:
\begin{align*}
R^\pi(T) & \ge T {\int_0^{\mu_{1-\varepsilon}} \mathbb{E}^\tau[N_\mu](\mu_{1-\varepsilon}-\mu)\zeta(d\mu)  \over \int_0^1 \mathbb{E}^\tau[N_\mu]\zeta(d\mu) }.
\end {align*}
To lower bound the numerator, we apply (\ref{eq:low2}) with $\mu_1=\mu_{1-{3\over 4}\varepsilon}$ and $\mu_2=\mu$. We obtain:
\begin{align*}
\int_0^{\mu_{1-\varepsilon}}  &\mathbb{E}^\tau[N_\mu](\mu_{1-\varepsilon}-\mu)\zeta(d\mu)\\
& \ge \int_0^{\mu_{1-\varepsilon}} \mathbb{E}^\tau[N_{\mu_{1-{3\over 4}\varepsilon}}](\mu_{1-\varepsilon}-\mu){\psi(\mu_{1-{3\over 4}\varepsilon},\mu)\over m}\zeta(d\mu).
\end{align*}
The denominator is upper bounded using (\ref{eq:low2}) again, and $\mathbb{E}^\tau[N_\mu]\le m$:
\begin{align*}
\int_0^1 \mathbb{E}^\tau[N_\mu]\zeta(d\mu) \le (1-{3\over 4}\varepsilon)\mathbb{E}^\tau[N_{\mu_{1-{3\over 4}\varepsilon}}]+{3\over 4}\varepsilon m.
\end{align*}
We conclude that: $R^\pi(T)\ge R_{\mathrm{ic}}(T)$ with
$$
R_{\mathrm{ic}}(T):= {T\over 2m} \int_0^{\mu_{1-\varepsilon}} (\mu_{1-\varepsilon}-\mu)\psi(\mu_{1-{3\over 4}\varepsilon},\mu)\zeta(d\mu).
$$
\ep

\subsection{Clustered items and clustured users}

To state regret lower bounds in this scenario, we introduce the following notations. For any $\ell\in [L]$, let $k^\star(\ell)=\arg\max_kp_{k\ell}$ the best item cluster for a user in ${\cal U}_\ell$, and for $k\neq k^\star(\ell)$, $\Delta_{k\ell}=p_{k^\star(\ell)\ell}-p_{k\ell}$ the gap between items from cluster ${\cal I}_k$ and ${\cal I}_{k^\star(\ell)}$. Denote by ${\cal L}(k)=\{\ell: k\in \arg\max_jp_{j\ell}\}$. We finally introduce the function:
$$
\phi(k,\ell,m,p) = {1\over 8} e^{-\gamma(p_{k^\star(\ell)\ell},p_{k\ell})}\times {1- e^{-m \gamma(p_{k^\star(\ell)\ell},p_{k\ell})}\over 1- e^{-\gamma(p_{k^\star(\ell)\ell},p_{k\ell})}}.
$$

Compared to the case of clustered items and statistically identical users, this scenario requires the algorithm to actually cluster users. This requirement induces an additional regret, denoted by $R_{\mathrm{uc}}(T)$ in the following theorem.

\begin{theorem}\label{th:lowC}
Let $\pi\in \Pi$ be an arbitrary algorithm. Then its regret satisfies: for all $T\ge m$ such that $m\ge c/\min_{k,\ell}\Delta_{k\ell}^2$ (for some constant $c$ large enough),
$$
R^\pi(T) \ge \max\{ R_{\mathrm{nr}}(T), R_{\mathrm{ic}}(T),R_{\mathrm{uc}}(T) \},
$$
where $R_{\mathrm{nr}}(T)$, $R_{\mathrm{ic}}(T)$, and $R_{\mathrm{uc}}(T)$ are the regrets due to the no-repetition constraint, to the unknown item clusters, and to the unknown user clusters respectively, defined by:
$$
\left\{
\arraycolsep=1.2pt\def\arraystretch{1.9}
\begin{array}{l}
R_{\mathrm{nr}}(T) = \mathbb{E}[\max_uN_u(T)] \sum_\ell\beta_\ell \sum_{k\neq k^\star(\ell)}\alpha_k\Delta_{k\ell},\\
R_{\mathrm{ic}}(T) = {T\over m} \sum_\ell\beta_\ell\sum_{k\neq k^\star(\ell)}\alpha_k \phi(k,\ell,m,p)\Delta_{k\ell},\\
R_{\mathrm{uc}}(T) = m(1-e^{-{T\over m}})\min_k(\sum_{\ell\notin {\cal L}(k)}\beta_\ell\Delta_{k\ell}).
\end{array}
\right.
$$
\end{theorem}

Note that we do not include in the lower bound the term $R_{\mathrm{uc}}(T)$ corresponding to the regret induced by the lack of knowledge of the success probabilities. Indeed, it would scale as $\log(T)$, and should $\min_k(\sum_{\ell\notin {\cal L}(k)}\beta_\ell\Delta_{k\ell})>0$, this regret would be negligible compared to $R_{\mathrm{uc}}(T)$ (remember that $T=o(m^2)$). 

The condition $\min_k(\sum_{\ell\notin {\cal L}(k)}\beta_\ell\Delta_{k\ell})>0$ just states that there is no item cluster that would be optimal for all users. Under this condition, the main component of regret is for all time horizon, small, medium, and large, is due to the unknown user clusters. The regret scales at least as $m$.    

{\bf Proof.} The proof of $R^\pi(T) \ge \max\{ R_{\mathrm{nr}}(T), R_{\mathrm{ic}}(T)\}$ is the same as in that of Theorem \ref{th:lowA}. To prove that $R^\pi(T) \ge R_{\mathrm{uc}}(T)$, assume that a user not encountered arrives. If we recommend an item of cluster $k$, we would suffer an average regret $\sum_{\ell\notin {\cal L}(k)}\beta_\ell\Delta_{k\ell}$ (since the user is of cluster ${\cal U}_\ell$ w.p. $\beta_\ell$. \ep  









  


==> lower3.tex <==
\section{Regret Lower Bounds}\label{sec:lower}


In this section, we derive regret lower bounds for the different structured problems introduced in the previous section. Interestingly, we are able to quantify the minimal regret induced by the specific and individual features of the problem: (i) the no-repetition constraint, (ii) the unknown success probabilities, (iii) the unknown item clusters, (iv) the unknown user clusters. 

\subsection{Clustered items and statistically identical users}

Recall that the success rates $p$ of the different clusters are such that $p_1>p_2\ge p_3\ge \ldots \ge p_K$. We denote by $\Delta_k=p_1-p_k$ the gap between items from the best cluster and items from cluster ${\cal I}_k$. We also introduce the function:
$$
\phi(k,m,p) = {1\over 8} e^{-\gamma(p_1,p_{k})}\times {1- e^{-m \gamma(p_1,p_{k})}\over 1- e^{-\gamma(p_1,p_{k})}},
$$
where $\gamma(p,q)=\kl(p,q)+\kl(q,p)$. Using the fact that $\kl(p,q)\le {(p-q)^2/ q(1-q)}$, we can easily show that as $m$ grows large, $\phi(k,m,p)$ scales as $\eta/(16\Delta_k^2)$ when $\Delta_k$ is small, where $\eta:=\min_kp_k(1-p_k)$. 

We aim at deriving problem-specific rather than minimax regret lower bounds, and as in the classical stochastic bandit literature, we hence need to introduce the notion of {\it uniformly} good algorithm. $\pi$ is uniformly good if its expected regret $R^\pi(T)$ is $O(\max\{ \sqrt{T}, {\log(m)\over \log({m\log(m)\over T}+e)})$ for all possible system parameters $(p,\alpha)$ when $T,m,n$ grows large with $T=o(nm)$ and $m\ge n$. In the next section, we establish that our proposed algorithms are uniformly good. 

\begin{theorem}\label{th:lowA}
Let $\pi\in \Pi$ be an arbitrary algorithm. Then its regret satisfies: for all $T\ge 1$ such that $m\ge c/\Delta_2^2$ (for some constant $c$ large enough),
$$
R^\pi(T) \ge \max\{ R_{\mathrm{nr}}(T), R_{\mathrm{ic}}(T) \},
$$
where $R_{\mathrm{nr}}(T)$ and $R_{\mathrm{ic}}(T)$ are the regrets due to the no-repetition constraint and to the unknown item clusters, respectively, defined by:
$$
\left\{
\arraycolsep=1.2pt\def\arraystretch{1.9}
\begin{array}{l}
R_{\mathrm{nr}}(T) = \mathbb{E}[\max_uN_u(T)]  \sum_{k\neq 1}\alpha_k\Delta_k,\\
R_{\mathrm{ic}}(T) = {T\over m} \sum_{k\neq 1}\alpha_k \phi(k,m,p)\Delta_k.
\end{array}
\right.
$$

Assume that $\pi$ is uniformly good, then we have\footnote{We write $a\gtrsim b$ if $\lim\inf_{T\to\infty}a/b\ge 1$.}:
$$
R^\pi(T)\gtrsim  R_{\mathrm{sp}}(T):=\log(T) \sum_{k\neq 1} {\Delta_k\over \kl (p_k,p_1)},
$$
where $R_{\mathrm{sp}}(T)$ refers to the regret due to the unknown success probabilities.
\end{theorem}

Before proving the theorem, let us see how the regret lower bounds scale for small, medium and large time horizons.

({\it Small horizon}) For $T=o(m\log(m))$, we get $R_{\mathrm{nr}}(T)=\Omega({\log(m)\over \log({m\log(m)\over T})})=\omega({T\over m})=\omega(R_{\mathrm{ic}}(T))$, and $R_{\mathrm{sp}}(T)=\Omega(\log(T))$. The regret arises mainly due to either the no-repetition constraint or the need to learn the success probabilities, depending on the relative values of ${\log(m)\over \log({m\log(m)\over T})}$ and $\log(T)$. For example, when $T=m$, the regret scales at least as $\log(T)$, but in general at least as  $\max\{ {\log(m)\over \log({m\log(m)\over T})}, \log(T)\}$. 

({\it Medium horizon}) For $T=c m\log(m)$, we get $R_{\mathrm{nr}}(T)=\Omega(\log(T))$, $R_{\mathrm{ic}}(T)=\Omega(\log(m))$, $R_{\mathrm{sp}}(T)=\Omega(\log(T))$. The three components of the regret lower bound scales in the same way, and the regret scales at least as $\log(T)$. 
 
({\it Large horizon}) For $T=\omega(m\log(m))$, we get $R_{\mathrm{nr}}(T)=\Omega({T\over m})$, $R_{\mathrm{ic}}(T)=\Omega({T\over m})$, $R_{\mathrm{sp}}(T)=\Omega(\log(T))$. One can easily check that ${T\over m}=\omega(\log(T))$, and hence learning the success probabilities induces a regret negligible compared to that due to the need to learn the item clusters or to deal with the no-repetition constraint. The regret then scales at least as ${T\over m}$.   

{\bf Proof.} Let $\pi\in \Pi$. We first establish that for any $T\ge 1$, $R^\pi(T) \ge R_{\mathrm{nr}}(T)$. Observe that under the no-repetition constraint, the number of items that $\pi$ will select is greater than $\max_uN_u(T)$. Now when an item is selected for the first time, by assumption, it belongs to the sub-optimal cluster ${\cal I}_k$ with probability $\alpha_k$, in which case this initial selection induces an expected regret $\Delta_k=p_1-p_k$. Hence indeed, $R^\pi(T) \ge \mathbb{E}[\max_uN_u]  \sum_{k\neq 1}\alpha_k\Delta_k$.

Next, we prove that $R^\pi(T) \gtrsim R_{\mathrm{sp}}(T)$. This part of the regret arises due to the lack of knowledge of the $p_k$'s. Assume that item clusters are known to the algorithm. The item selection problem reduces to a classical stochastic bandit problem. Using the techniques developed in  \cite{lai1985asymptotically} and recently extended in \cite{garivier2018explore}, we can prove that $R^\pi(T) \gtrsim \log(T) \sum_{k\neq 1} {\Delta_k\over \kl (p_k,p_1)}$. Note that here, we scale the time horizon and the number items (arms) simultaneously, which requires finite-time arguments as those developed in \cite{garivier2018explore}. Refer to the appendix for a complete proof.

Finally, the most involved part of the proof is to lower bound the regret due to the lack of knowledge of the item clusters, i.e., to prove that for $T\ge 1$, $R^\pi(T)\ge R_{\mathrm{ic}}(T)$. To this aim, assume that the success probabilities $p_k$'s are known. Further simplify the problem by relaxing the no-repetition constraint: instead, we just impose that any item cannot be selected more than $m$ times. With these assumptions, an optimal algorithm can be described through a simple stopping rule $\tau$. When a new item is selected, $\tau$ decides whether to select this item further depending on its previously observed rewards. when $\tau$ decides to stop exploring the item, a new item is selected. Let $\mathbb{E}^\tau[N_k]$ denote the expected number of times an item of cluster ${\cal I}_k$ is selected under $\tau$ (of course, $N_k\le m$). The next lemma is the main ingredient of the proof.

\begin{lemma}\label{lem:2arms} We have for any $m\ge c/\Delta_2^2$ and for any $k\neq 1$:      
$$
{\phi(k,m,p)\over m}\le {\mathbb{E}^\tau[N_k]\over \mathbb{E}^\tau[N_{1}]} \le 1.
$$
\end{lemma}

The constant $c$ in the above lemma is the same as in Theorem \ref{th:lowA}, and is chosen such that when $m\ge c/\Delta_2^2$, then for any $k$, $\phi(k,m,p)\le m$. This choice ensures that the inequality stated in the above lemma makes sense (we know that $\mathbb{E}^\tau[N_k]\le m$).

{\it Proof of Lemma \ref{lem:2arms}.} This results is proved considering a 2-arm bandit problem. The arms have Bernoulli rewards with respective means $p_1$ and $p_k$. The means are known but the arm with the highest mean is unknown. For this bandit problem, we can build an algorithm based on our stopping rule $\tau$ in the following way: we initially pick an arm uniformly at random and play it using the stopping rule $\tau$; we then switch arm and repeat (when we switch to an arm already played in the past, the previous rewards are discarded). We stop the algorithm when we have switched an odd number of times and the number of rounds is larger than $m$. Let $\kappa$ denote the number of stopping rules applied to the two arms. $\kappa$ is a random variable, and Wald's first lemma implies that the regret accumulated before we stop playing is:
$
R^\tau = \Delta_k \mathbb{E}[\kappa]\mathbb{E}^\tau[N_k].
$
Since $\max\{\mathbb{E}^\tau[N_1],\mathbb{E}^\tau[N_k]\}\le m$, $\mathbb{E}[\kappa]\mathbb{E}^\tau[N_{1}]\le 2m$. Hence:
\begin{equation}\label{eq:reg1}
R^\tau = \Delta_k \mathbb{E}[\kappa]\mathbb{E}^\tau[N_k]\le 2m \Delta_k {\mathbb{E}^\tau[N_k]\over \mathbb{E}^\tau[N_{1}]}.
\end{equation}
Observe that by construction, $R^\tau$ corresponds to the regret of our algorithm for a number of rounds larger than $m$ in the 2-arm bandit problem with known average rewards. Regret lower bounds for such bandit problems have been derived in \cite{Bubeck13}. We can actually show that (refer to the appendix for a proof):

\begin{lemma}\label{lem:reg-2arm} We have: $R^\tau \ge {\Delta_k}\phi(k,m,p)$.
\end{lemma}

Combining this lemma to (\ref{eq:reg1}) yields Lemma \ref{lem:2arms}. \ep

We complete the proof of $R^\pi(T)\ge R_{\mathrm{ic}}(T)$ using Lemma \ref{lem:2arms}. We use our optimal stopping rule $\tau$ for the simplified problem where the $p_k$'s are known, and where the no-repetition constraint is simplified. Each time a new item is selected, it belongs to ${\cal I}_k$ w.p. $\alpha_k$ and it is played $\mathbb{E}^\tau[N_k]$ in expectation. Thus, the expected regret per round of our optimal algorithm is: ${\sum_{k\neq 1} \alpha_k \mathbb{E}^\tau[N_k]\Delta_k\over \sum_{k} \alpha_k \mathbb{E}^\tau[N_1]}$. We conclude that:
\begin{align*}
R^\pi(T) & \ge T {\sum_{k\neq 1} \alpha_k \mathbb{E}^\tau[N_k]\Delta_k\over \sum_{k} \alpha_k \mathbb{E}^\tau[N_k]}\\
&  \stackrel{(a)}{\ge} {T\over m} {\sum_{k\neq 1} \alpha_k \mathbb{E}^\tau[N_1]\phi(k,m,p)\Delta_k \over \sum_{k} \alpha_k \mathbb{E}^\tau[N_1]}\\
& = {T\over m} \sum_{k\neq 1}\alpha_k \phi(k,m,p)\Delta_k,
\end {align*}
where the inequality (a) stems from applying Lemma \ref{lem:2arms} (in the numerator, we use $\mathbb{E}^\tau[N_k]\ge \mathbb{E}^\tau[N_1]{\phi(k,m,p)\over m}$, and in the denominator $\mathbb{E}^\tau[N_k]\le \mathbb{E}^\tau[N_1]$). \ep 

\subsection{Unclustered items and statistically identical users}

In this scenario, the regret of an algorithm is induced by the no-repetition constraint and by the fact the success rate of an item when it is first selected is unknown (even if the a-priori distribution $\zeta$ could be known). These two sources of regret lead to the terms  
$R_{\mathrm{nr}}(T)$ and $R_{\mathrm{ic}}(T)$, respectively, in our regret lower bound.

\begin{theorem}\label{th:lowB}
Assume that the density of $\zeta$ satisfies, for some $C>0$, $\zeta(\mu) \le C$ for all $\mu\in [0,1]$. Let $\pi\in \Pi$ be an arbitrary algorithm. Then its regret satisfies: for all $T\ge 1$ such that $m\ge c/\varepsilon^2$ (for some constant $c\ge 1$ large enough),
$$
R_\varepsilon^\pi(T) \ge \max\{ R_{\mathrm{nr}}(T), R_{\mathrm{ic}}(T) \},
$$
where $R_{\mathrm{nr}}(T)$ and $R_{\mathrm{ic}}(T)$ are defined by:
$$
\left\{
\arraycolsep=1.2pt\def\arraystretch{1.9}
\begin{array}{l}
R_{\mathrm{nr}}(T) = \mathbb{E}[\max_uN_u(T)]  \int_0^{\mu_{1-\varepsilon}} (\mu_{1-\varepsilon}-\mu)\zeta(\mu)d\mu,\\
R_{\mathrm{ic}}(T) = {T\over m} {(1-\varepsilon)^2/(2C)  \over \min\{ 1, (1+C)\varepsilon \}  + 1/m}.
\end{array}
\right.
$$
\end{theorem}

{\bf Proof.} We apply the same strategy to derive regret lower bound in the case of clustered items. Regarding the regret induced by the no-repetition constraint, we simply get:
$$
R_{\mathrm{nr}}(T) = \mathbb{E}[\max_uN_u(T)]  \int_0^{\mu_{1-\varepsilon}} (\mu_{1-\varepsilon}-\mu)\zeta(\mu)d\mu.
$$
For the term $R_{\mathrm{ic}}(T)$, assume that $\zeta$ is known. The optimal algorithm boils down to a stopping rule $\tau$ that aims at deciding whether the current item has a success rate greater than $\mu_{1-\varepsilon}$. We denote by $\mathbb{E}^\tau[N_\mu]$ the expected number of rounds an item with success rate $\mu$ is selected under $\tau$.

Now the regret of an algorithm $\pi$ satisfies:
\begin{align*}
R_\varepsilon^\pi(T) & \ge T {\int_0^{\mu_{1-\varepsilon}} \mathbb{E}^\tau[N_\mu](\mu_{1-\varepsilon}-\mu)\zeta(\mu)d\mu  \over \int_0^1 \mathbb{E}^\tau[N_\mu]\zeta(\mu)d\mu } \cr
& \ge T {\int_0^{\mu_{1-\varepsilon}} \mathbb{E}^\tau[N_\mu](\mu_{1-\varepsilon}-\mu)\zeta(\mu)d\mu  \over \min\{ 1, (1+C)\varepsilon \} m + \int_0^{\mu_{1-\varepsilon} -\varepsilon} \mathbb{E}^\tau[N_\mu]\zeta(\mu)d\mu } \cr
& \ge T {(1-\varepsilon)^2/(2C)  \over \min\{ 1, (1+C)\varepsilon \} m + 1},
\end {align*}
where we use the fact that $\varepsilon \ge \frac{1}{\sqrt{m}}$ and  $1\le \mathbb{E}^\tau[N_\mu] \le m$ for all $\mu$. The last inequality is obtained by remarking that for $\mu\le \mu_{1-\varepsilon}-\varepsilon$, the function ${\int_0^{\mu_{1-\varepsilon}} \mathbb{E}^\tau[N_\mu](\mu_{1-\varepsilon}-\mu)\zeta(d\mu)  \over \min\{ 1, (1+C)\varepsilon \} m + \int_0^{\mu_{1-\varepsilon} -\varepsilon} \mathbb{E}^\tau[N_\mu]\zeta(d\mu) }$ is either increasing or decreasing in $\mathbb{E}^\tau[N_\mu]$, depending on $\mu$. We can hence derive a lower bound of this function by investigating extreme scenarios where $\mathbb{E}^\tau[N_\mu]$ is 1 or $+\infty$. More precisely, if the $\zeta$-measure of the set of $\mu\in [0,\mu_{1-\varepsilon}-\varepsilon]$ such that the function is decreasing is strictly positive, by setting $\mathbb{E}^\tau[N_\mu]$ to $+\infty$ to the $\mu$'s in this set, we get that the function is lower bounded $1/\varepsilon$. Otherwise, we set $\mathbb{E}^\tau[N_\mu]=1$ to all $\mu$'s, and get the lower bound ${(1-\varepsilon)^2/(2C)  \over \min\{ 1, (1+C)\varepsilon \} m + 1}$. The proof of is completed by noticing that ${(1-\varepsilon)^2/(2C)  \over \min\{ 1, (1+C)\varepsilon \} m + 1}\le 1/\varepsilon$. \ep

\subsection{Clustered items and clustured users}

To state regret lower bounds in this scenario, we introduce the following notations. For any $\ell\in [L]$, let $k^\star(\ell)=\arg\max_kp_{k\ell}$ the best item cluster for a user in ${\cal U}_\ell$, and for $k\neq k^\star(\ell)$, $\Delta_{k\ell}=p_{k^\star(\ell)\ell}-p_{k\ell}$ the gap between items from cluster ${\cal I}_k$ and ${\cal I}_{k^\star(\ell)}$. Denote by ${\cal L}(k)=\{\ell: k\in \arg\max_jp_{j\ell}\}$. We finally introduce the function:
$$
\phi(k,\ell,m,p) = {1\over 8} e^{-\gamma(p_{k^\star(\ell)\ell},p_{k\ell})}\times {1- e^{-m \gamma(p_{k^\star(\ell)\ell},p_{k\ell})}\over 1- e^{-\gamma(p_{k^\star(\ell)\ell},p_{k\ell})}}.
$$

Compared to the case of clustered items and statistically identical users, this scenario requires the algorithm to actually cluster users. This requirement induces an additional regret, denoted by $R_{\mathrm{uc}}(T)$ in the following theorem.

\begin{theorem}\label{th:lowC}
Let $\pi\in \Pi$ be an arbitrary algorithm. Then its regret satisfies: for all $T\ge m$ such that $m\ge c/\min_{k,\ell}\Delta_{k\ell}^2$ (for some constant $c$ large enough),
$$
R^\pi(T) \ge \max\{ R_{\mathrm{nr}}(T), R_{\mathrm{ic}}(T),R_{\mathrm{uc}}(T) \},
$$
where $R_{\mathrm{nr}}(T)$, $R_{\mathrm{ic}}(T)$, and $R_{\mathrm{uc}}(T)$ are the regrets due to the no-repetition constraint, to the unknown item clusters, and to the unknown user clusters respectively, defined by:
$$
\left\{
\arraycolsep=1.2pt\def\arraystretch{1.9}
\begin{array}{l}
R_{\mathrm{nr}}(T) = \mathbb{E}[\max_uN_u(T)] \sum_\ell\beta_\ell \sum_{k\neq k^\star(\ell)}\alpha_k\Delta_{k\ell},\\
R_{\mathrm{ic}}(T) = {T\over m} \sum_\ell\beta_\ell\sum_{k\neq k^\star(\ell)}\alpha_k \phi(k,\ell,m,p)\Delta_{k\ell},\\
R_{\mathrm{uc}}(T) = m(1-e^{-{T\over m}})\min_k(\sum_{\ell\notin {\cal L}(k)}\beta_\ell\Delta_{k\ell}).
\end{array}
\right.
$$
\end{theorem}

Note that we do not include in the lower bound the term $R_{\mathrm{uc}}(T)$ corresponding to the regret induced by the lack of knowledge of the success probabilities. Indeed, it would scale as $\log(T)$, and should $\min_k(\sum_{\ell\notin {\cal L}(k)}\beta_\ell\Delta_{k\ell})>0$, this regret would be negligible compared to $R_{\mathrm{uc}}(T)$ (remember that $T=o(m^2)$). 

The condition $\min_k(\sum_{\ell\notin {\cal L}(k)}\beta_\ell\Delta_{k\ell})>0$ just states that there is no item cluster that would be optimal for all users. Under this condition, the main component of regret is for all time horizon, small, medium, and large, is due to the unknown user clusters. The regret scales at least as $m$.    

{\bf Proof.} The proof of $R^\pi(T) \ge \max\{ R_{\mathrm{nr}}(T), R_{\mathrm{ic}}(T)\}$ is the same as in that of Theorem \ref{th:lowA}. To prove that $R^\pi(T) \ge R_{\mathrm{uc}}(T)$, assume that a user not encountered arrives. If we recommend an item of cluster $k$, we would suffer an average regret $\sum_{\ell\notin {\cal L}(k)}\beta_\ell\Delta_{k\ell}$ (since the user is of cluster ${\cal U}_\ell$ w.p. $\beta_\ell$). Then, in $T$ rounds, the number of users arriving is in expectation $m(1-(1-{1\over m})^T)\ge m(1-e^{T/m})$.\ep  









  

